Lost in Literalism: How Supervised Training Shapes Translationese in LLMs

Large language models (LLMs) have achieved remarkable success in machine translation, demonstrating impressive performance across diverse languages. However, translationese, characterized by overly literal and unnatural translations, remains a persistent challenge in LLM-based translation systems. Despite their pre-training on vast corpora of natural utterances, LLMs exhibit translationese errors and generate unexpected unnatural translations, stemming from biases introduced during supervised fine-tuning (SFT). In this work, we systematically evaluate the prevalence of translationese in LLM-generated translations and investigate its roots during supervised training. We introduce methods to mitigate these biases, including polishing golden references and filtering unnatural training instances. Empirical evaluations demonstrate that these approaches significantly reduce translationese while improving translation naturalness, validated by human evaluations and automatic metrics. Our findings highlight the need for training-aware adjustments to optimize LLM translation outputs, paving the way for more fluent and target-language-consistent translations. We release the data and code at https://github.com/yafuly/LLM_Translationese.

==> bkp.tex <==
\begin{table*}
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
% \begin{spacing}{1.0}
\begin{CJK*}{UTF8}{gbsn}
\resizebox{\textwidth}{!}{\begin{tabular}{cc}
\toprule
\multicolumn{2}{c}{\textbf{Sentence-level Translationese}} \\
\midrule
\multirow{2}{*}{\textbf{Source}: Few-shot LMs still lag behind vanilla fine-tuned models in the task.} & \textbf{LLM}: 少量样本LMs仍然落后于原始细化训练模型在任务中。 \\
 & \textbf{Human}: 在任务中，少样本LMs仍然落后于原始细化训练模型。 \\
 \\
 \multirow{2}{*}{\textbf{Source}: Bei starker Hitze ließ diese Festigkeit zwar etwas nach.} & \textbf{LLM}: However, at high temperatures this hardness did diminish somewhat. \\
 & \textbf{Human}: However, the hardness diminished somehow at high temperatures. \\

\midrule
 \multicolumn{2}{c}{\textbf{Phrase-level Translationese}} \\
\midrule
\multirow{2}{*}{\textbf{Source}: ffter a quick trip in the microwave} & \textbf{LLM}: 在微波炉的快速旅行后 \\
 & \textbf{Human}: 在微波炉中快速加热后 \\
 \\
 \multirow{2}{*}{\textbf{Source}: mehr Lebensqualität zu gewinnen} & \textbf{LLM}: gain more quality of life \\
 & \textbf{Human}: improve living standards \\
\bottomrule
\end{tabular}}
% \end{spacing}
\caption{
\label{translation_engine}
Examples of sentence-level and phrase-level translationese, with each one presenting an English-to-Chinese translation and a German-to-English translation.
}
% \footnote{https://translate.google.cn/}
\end{CJK*}
\end{table*}




\begin{table}
\centering
\small
% \setlength{\tabcolsep}{2.5pt}
% \begin{spacing}{1.0}
\renewcommand{\arraystretch}{1.35}
\begin{CJK*}{UTF8}{gbsn}
\resizebox{0.48\textwidth}{!}{\begin{tabular}{cc}
\toprule
\multicolumn{2}{c}{\textbf{Sentence-level Translationese}} \\
\midrule
\textbf{Source} & Few-shot LLMs still lag behind vanilla fine-tuned models \textcolor{blue}{in the task}. \\
\textbf{LLM} & 少量样本LLMs仍然落后于原始细化训练模型\textcolor{red}{在任务中}。 (ppl: 151.5) \\
 \textbf{Refine} & \textcolor{red}{在任务中}，少样本LLMs仍然落后于原始细化训练模型。 (ppl: 128.8) \\
\textbf{Source} & \textcolor{blue}{Bei starker Hitze} ließ diese Festigkeit zwar etwas nach.\\
\textbf{LLM} &  However, \textcolor{red}{at high temperatures} this hardness did diminish somewhat. (ppl: 160.1) \\
\textbf{Refine}  &  However, this hardness did diminish somewhat \textcolor{red}{at high temperatures}.  (ppl: 96.6)\\
\midrule

\multicolumn{2}{c}{\textbf{Phrase-level Translationese}} \\
\midrule
\textbf{Source} & \textcolor{blue}{after a quick trip} in the microwave \\
\textbf{LLM} & 在微波炉\textcolor{red}{的快速旅行后} (ppl: 394.3) \\
 \textbf{Refine} & 在微波炉\textcolor{red}{中快速加热后} (ppl: 56.3) \\
\textbf{Source} & \textcolor{blue}{mehr Lebensqualität zu gewinnen}\\
\textbf{LLM} &  \textcolor{red}{gain more quality of life}  (ppl: 620.5)\\
\textbf{Refine}  &  \textcolor{red}{improve living standards} (ppl: 368.8)\\
\bottomrule
\end{tabular}}
% \end{spacing}
\caption{
\label{translation_engine}
Examples of Sentence-level and Phrase-level Translationese: This table presents translation cases from English-to-Chinese and German-to-English. Each case includes an LLM-generated translation alongside a refined version, with perplexity (PPL) values provided at the end. \textcolor{blue}{Blue} text highlights the source segments, while \textcolor{red}{red} text identifies segments in the LLM translation where translationese occurs and is subsequently refined.
}
\end{CJK*}
\end{table}



\begin{table}
\centering
\footnotesize
% \setlength{\tabcolsep}{2.5pt}
% \begin{spacing}{1.0}
\renewcommand{\arraystretch}{1.1}
\begin{CJK*}{UTF8}{gbsn}
\resizebox{0.5\textwidth}{!}{\begin{tabular}{cc}
\toprule
\multicolumn{2}{c}{\textbf{Sentence-level Translationese}} \\
\midrule
\multirow{2}{*}{\textbf{Source}} & Few-shot LLMs still lag behind vanilla \\
& fine-tuned models \textcolor{blue}{in the task}. \\
\multirow{2}{*}{\textbf{LLM}} & 少量样本LLMs仍然落后于原始 \\
& 细化训练模型\textcolor{red}{在任务中}。 (ppl: 151.5) \\
 \multirow{2}{*}{\textbf{Refine}} & \textcolor{red}{在任务中}，少样本LLMs仍然落后于原始 \\
 & 细化训练模型。 (ppl: 128.8) \\
 \hline
 \multirow{2}{*}{\textbf{Source}} & \textcolor{blue}{Bei starker Hitze} ließ diese Festigkeit \\
 & zwar etwas nach.\\
 \multirow{2}{*}{\textbf{LLM}} &  However, \textcolor{red}{at high temperatures} this hardness \\
 & did diminish somewhat. (ppl: 160.1) \\
 \multirow{2}{*}{\textbf{Refine}}  &  However, this hardness did diminish \\
 & somewhat \textcolor{red}{at high temperatures}.  (ppl: 96.6)\\
\midrule

\multicolumn{2}{c}{\textbf{Phrase-level Translationese}} \\
\midrule
\textbf{Source} & \textcolor{blue}{after a quick trip} in the microwave \\
\textbf{LLM} & 在微波炉\textcolor{red}{的快速旅行后} (ppl: 394.3) \\
 \textbf{Refine} & 在微波炉\textcolor{red}{中快速加热后} (ppl: 56.3) \\
 \hline
\textbf{Source} & \textcolor{blue}{mehr Lebensqualität zu gewinnen}\\
\textbf{LLM} &  \textcolor{red}{gain more quality of life}  (ppl: 620.5)\\
\textbf{Refine}  &  \textcolor{red}{improve living standards} (ppl: 368.8)\\
\bottomrule
\end{tabular}}
% \end{spacing}
\caption{
\label{translation_engine}
Examples of Sentence-level and Phrase-level Translationese: This table presents translation cases from English-to-Chinese and German-to-English. Each case includes an LLM-generated translation alongside a refined version, with perplexity (PPL) values provided at the end. \textcolor{blue}{Blue} text highlights the source segments, while \textcolor{red}{red} text identifies segments in the LLM translation where translationese occurs and is subsequently refined.
}
\end{CJK*}
\end{table}


==> tables/compare_polish.tex <==
\begin{table}[t]
% \setlength{\belowcaptionskip}{-0.4cm}
\centering
\small
% \setlength{\tabcolsep}{10pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.2}
\begin{tabular}{ccccc}
\toprule
\multirow{2}{*}{\textbf{Training}} &\multicolumn{2}{c}{\textbf{Llama3.1-8B}}  & \multicolumn{2}{c}{\textbf{Qwen2.5-7B}}\\
& \textbf{En-Zh} & \textbf{De-En} & \textbf{En-Zh} & \textbf{De-En} \\ 
 \midrule
 % \multicolumn{}{c}{Llama3.1-8B}  \\
 % \midrule
SFT  & 80.0  & 80.5 & 73.8 & 74.0\\
w/ Post-polish & 81.5  & \textbf{81.2} & \textbf{74.7} & 75.3\\
SFT-Polish & \textbf{81.8} & 81.0  & 74.2 & \textbf{75.6}\\
% \hline
\bottomrule
\end{tabular}
% \vspace{-0.2cm}
\caption{}
\label{tab:compare_post_polish}
\end{table}

